No Pairs Left Behind: Improving Metric Learning with Regularized Triplet Objective

We propose a novel formulation of the triplet objective function that improves metric learning without additional sample mining or overhead costs. Our approach aims to explicitly regularize the distance between the positive and negative samples in a triplet with respect to the anchor-negative distance. As an initial validation, we show that our method (called No Pairs Left Behind [NPLB]) improves upon the traditional and current state-of-the-art triplet objective formulations on standard benchmark datasets. To show the effectiveness and potentials of NPLB on real-world complex data, we evaluate our approach on a large-scale healthcare dataset (UK Biobank), demonstrating that the embeddings learned by our model significantly outperform all other current representations on tested downstream tasks. Additionally, we provide a new model-agnostic single-time health risk definition that, when used in tandem with the learned representations, achieves the most accurate prediction of subjects' future health complications. Our results indicate that NPLB is a simple, yet effective framework for improving existing deep metric learning models, showcasing the potential implications of metric learning in more complex applications, especially in the biological and healthcare domains.

==> Methods/HRDef.tex <==
\subsection{Definition of Health Risk from a Single Visit}
\label{sec:methods-HR}
 In this section, we aim to provide a mathematical definition of health risk that can measure similarity between a new cohort and an existing \bone healthy population without requiring temporal data. This definition is inspired by the formulation of risk in other domains, such as defining the risk of re-identification of anonymized data \cite{Risk-AnonData}. We first define the notion of a "health distance", and use that to formulate thresholds intervals which enable us a define health risk as a mapping between continuous values and discrete risk groups. 

\begin{definition}
\label{def:healthScore}
Given a space $X$, a \bone healthy population distribution $B$ and a new patient $p$ (all in $X$), the \textbf{health score} $s_n$ of $p$ is:
$$s_q(p) = d(P_q(B), p) $$
where $P_q(H)$ denotes the $q^{\text{th}}$ percentile of $B$, and $d(\cdot)$ refers to a metric defined on $X$ (potentially a pseudo metric).
\end{definition}

Definition \ref{def:healthScore} provides a measure of distance between a new patient and an existing reference population, which can be used to define similarity. For example, if $d(\cdot)$ is the Euclidean distance, then the similarity between patient $x$ and $y$ is $sim(x,y) = \frac{1}{1+d(x,y)}$. Next, using this notion of distance (and similarity), we define risk thresholds that allow for grouping of patients. 
\begin{definition}
\label{def:threshold}
A threshold interval $I_q = [t_q^l, t_q^u]$ is defined as the distance between the vectors providing the inner $q$ percent of a distribution $H$ and the median value. Let $n = (100-q)/2$, then we have $I_q$ as:
$$I_q = [t_q^l, t_q^u] =\left[d(P_{n}(H), P_{50}(H)),d(P_{q+n}(H), P_{50}(H))\right].$$
\end{definition}
\smallskip  
Additionally, for the sake of interpretability and convenience, we can define \textbf{health risk groups} using \emph{known} $I_q$ values which we define below.
\begin{definition}
\label{def:riskBukcets}
Let $M:\R^d \to V \cup \{\eta \}$ where $d$ denotes the number of features defining a patient, with $\eta$ being discrete group and $V$ denoting pre-defined risk groups based on $k\in \N$ many intervals (i.e. $|V|=|I_q|=k$). Using the same notion of health distance $s_n$ and threshold interval $I_q$ as before, we define a patient $p$'s health risk group as:
\begin{equation*}
    M(p) = 
    \begin{cases}
    V_q \hspace{3 mm} &\text{if} \hspace{2 mm}  s_q(p) \in I_q \\
    \eta \hspace{3 mm} &\text{otherwise} \\
    \end{cases}
    .
\end{equation*}
\end{definition}

We utilize this definition for constructing discrete health groups in Section \ref{sec:methods-prediction}.

\subsection{Predicting Health Risks from a Single Visit}
\label{sec:methods-prediction}

Now that we have presented our deep metric learning model and the definition of health risk from a single visit, we utilize these two in tandem to predict health risks. That is, we first produce embeddings for all patients using our learned nonlinear operator $G$, and then use the distance between the \bone healthy (BFH) population and new patients to assign them a risk group. Mathematically, given the set of BFH population for all groups, i.e. 
$$B_{All} = \{B_{[36,45]}, B_{[46,50]}, B_{[51,55]}, B_{[56,60]}, B_{[61,65]}, B_{[66,75]}\},$$ 
we take the reference value \textit{per age group} to be $$\tilde{r}_{age} = G(P_{50}(B_{age})),$$ where $B_{age}$ denotes the BFH population for the age group $age$. Then, using definition \ref{def:threshold}, we define:
\begin{subequations}
\begin{align}
    N_{age} = I_{95}^{age} = \left[d(P_{2.5}(B_{age}), P_{50}(B_{age})),d(P_{97.5}(B_{age}), P_{50}(B_{age}))\right]
\end{align}
\begin{align}
    LR_{age} = I_{98}^{age} = \left[d(P_{1}(B_{age}), P_{50}(B_{age})),d(P_{99}(B_{age}), P_{50}(B_{age}))\right].
\end{align}
\label{eq:intervals}
\end{subequations}
Note that $N_{age} \subset LR_{age}$. Lastly, using the intervals defined in Eq. \eqref{eq:intervals}, we define the mapping $M$ as shown in Eq. \eqref{eq:methods-riskmapping}.
\begin{equation}
    M_{age}(p)= 
    \begin{cases}
    \text{Normal} \hspace{3 mm} &\text{if} \hspace{2 mm} s_n(G(p)) = d(G(p),\tilde{r}_{age}) \in N_{age} \\
    \\
    \text{Lower Risk} \hspace{3 mm} &\text{if} \hspace{2 mm}  s_n(G(p))=d(G(p),\tilde{r}_{age}) \in LR_{age} \backslash N_{age}\\ 
    \\
    \text{Higher Risk} \hspace{3 mm} &\text{otherwise}
    \end{cases}
    .
    \label{eq:methods-riskmapping}
\end{equation}


==> Results/Results.tex <==
\subsection{Training Procedure and Architecture}
\label{sec:methods-arch}
Prior to training, we split the data $80\%:20\%$ for training and testing. In the training partition, we augment the \bone population 3 folds (described in Section \ref{sec:methods-augmenting}), and then generate 80K triplets of the form $(a_i, p_i, n_i)$ randomly in an offline manner. We chose to generate only 80K triplets in order to reduce training time and demonstrate the capabilities of our approach for smaller datasets. Note that in an unsupervised setting, these triplets need to be generated online via negative sample mining, but this is out of scope for this work given that we have labels \apriori. Our model consists of the three hidden layers with two probabilistic dropout layers in between and Parametric Rectified Linear Units (PReLU) \cite{PRelu} nonlinear activations. We present a visual representation of our architecture and the dimensions in Fig. \ref{fig:Appendix-NNArchitecture}. We optimize the weights for minimizing Eq.\eqref{eq:triplet-reg-2} function using Adam \cite{adam} for 1000 epochs with $lr=0.001$, and employ an exponential learning rate decay ($\gamma=0.95$) to decrease the learning rate after every 50 epochs. In order to test the true capability of our model, all evaluations are performed on the \emph{non-augmented} data. 


% Generally, there are two classes of interpretable methods \cite{classesOfModelInterpretibility}: The first group are methods where the model itself is explainable at an algorithmic level (e.g. linear regression or rule-based models); however, these models often become less interpretable as the complexity of the model increases,  and (ii) post-hoc interpretable algorithms which aim to provide insights on a models output and decision making process. Giv

\subsection{Augmenting \textit{Bona Fide} Healthy Population}
\label{sec:methods-augmenting}
Given the small number of the BFH samples compared to the other two populations, we experimented with the possibility of augmenting the data with generated BFH samples. In order to keep the DML-based as the main focus of this paper, we implemented a simple yet intuitive rejection-based sampling to generate synthetic BFH patients, though more sophisticated methods could be employed. Similar to any other rejection-based sampling, we construct a surrogate probability distribution $P(x_i)$ for each feature $x_i$ across all patients; based on empirical results and as a common assumption \cite{LabWorkNormalDistribution}, we assumed that each feature is a Gaussian $\mathcal{N}(\mu_x, \sigma_x)$ where $\mu_x$ and $\sigma_x$ denote the empirical mean and standard deviation of feature $x_i$ for all patients. As noted earlier, a BFH patients is selected if their $P_0$ biosignals fall within the clinically-normal lab ranges. Therefore, it is an intuitive choice to use the bounds of the clinically normal range as the accept/reject criteria. Our simple rejection-based sampling scheme is presented in Algorithm \ref{alg:sampling}. 


We evaluate the performance of our deep metric learning model by quantitatively and qualitatively assessment of the embeddings in Section \ref{sec:results-classification}. Utilizing our definition of health risk, we predict general health risks for patients using a single lab visit, as presented in Section \ref{sec:results-risk}. Due to space constraints and the similarity between our findings, we present our findings on the \emph{female} population in the main manuscript, and provide the analysis of the male population in the Appendix.


% \subsection{Extracting Most Important Features}
% \label{sec:results-attention}
% \ali{Ali is working on feature permuation, PDP and Shapely values for this section.}
% % Analyzing SPHR's interpretability is possible by extracting top $n$ attention values (per feature) for each patient. The resulting features reflect SPHR learning to evaluate them . To evaluate, we extracted the top 10 fe

\subsection{Predicting Healthy Patient's Health Risks}
\label{sec:results-risk}
We utilized our single-time health risk definition to predict patient's future potentials of health complications. To demonstrate the versatility of our approach, we predicted \emph{general} health risks that were used for all health conditions available (namely \textit{Cancer, Diabetes and Other Serious Conditions}); however, we hypothesize that constraining health risks based on specific conditions will improve risk predictions. We considered five methods for assigning a risk group to each patient: (i) Euclidean distance on raw data (preprocessed but not transformed), (ii) Mahalanobis distance on pre-processed data, (iii) Euclidean distance on the key metrics ($P_0$) for the available conditions(described in section \ref{sec:data-ultraHealthy}), therefore hand-crafting features and reducing dimensionality in order to achieve an upper bound performance for most traditional methods (though this will not be possible for all diseases). The last two methods we consider are deep representation learning methods: (iv) DeepPatient and (v) SPHR embeddings (proposed model). We use the Euclidean metric for calculating the distance between deep-learned representations of (iv) and (v).

We evaluated the effectiveness of the methods in two-steps:
\begin{enumerate}
    \item We assessed the percentage of the apparently-healthy and unhealthy population that were assigned to the three health risk groups defined in Section \ref{sec:methods-prediction}. Our intuition here was that, given the continuum of patient's health status, a method that predicts all apparently-healthy individuals as "normal" is not a good predictor of future complications (and vice versa for the unhealthy group). We present these results in Table \ref{tab:GeneralHealthRiskPrediction}. 
    
    \item We assigned all patients to one of the three risk groups using a single visit. In order to validate the risk groups predicted, we retrieved all available next check ups from the UK Biobank, and calculated the percentage of patients who developed a condition in the next visit. We note that the future visits contained significantly fewer patients (up to 100x fewer in some cases). Intuitively, patients who fall under the "Normal" risk level should have fewer confirmed cases compared to subjects in "Lower Risk" or "Higher Risk" groups. Table \ref{tab:FutureRiskPrediction} shows the results for the top three methods, with our approach consistently matching the intuitive criteria: among the five methods, SPHR-predicted patients in the \textit{Normal} risk group have the fewest instance of developing future conditions, while the ones predicted as \textit{High} Risk have the highest instance of developing future conditions (shown in Table \ref{tab:FutureRiskPrediction}).
    
    \begin{table}[H]
\centering
\caption{\textbf{Percentage of patients assigned to each risk group per method.} For both the apparently healthy and unhealthy population, we calculated the percentage of subjects assigned to each risk group. Abbreviations: \textit{N}: Normal Risk, \textit{LR}: Lower Risk, \textit{HR}: Higher Risk.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|}
\cline{2-16}
\multicolumn{1}{c|}{\textbf{}}           & \multicolumn{3}{c|}{\textbf{Euclidean}}                                                            & \multicolumn{3}{c|}{\textbf{Mahalanobis}}                                        & \multicolumn{3}{c|}{\textbf{P0 Euclidean}}                                       & \multicolumn{3}{c|}{\textbf{DeepPatient}}                                        & \multicolumn{3}{c|}{\textbf{SPHR (Ours)}}                                               \\ \cline{2-16} 
\textit{}                                & \multicolumn{1}{c|}{\textit{N}}   & \multicolumn{1}{c|}{\textit{LR}}               & \textit{HR}   & \multicolumn{1}{c|}{\textit{N}} & \multicolumn{1}{c|}{\textit{LR}} & \textit{HR} & \multicolumn{1}{c|}{\textit{N}} & \multicolumn{1}{c|}{\textit{LR}} & \textit{HR} & \multicolumn{1}{c|}{\textit{N}} & \multicolumn{1}{c|}{\textit{LR}} & \textit{HR} & \multicolumn{1}{c|}{\textit{N}} & \multicolumn{1}{c|}{\textit{LR}} & \textit{HR} \\ \hline
\multicolumn{1}{|l|}{\textit{App. Healthy}}       & \multicolumn{1}{c|}{97\%}         & \multicolumn{1}{c|}{1.5\%}                     & 1.5\%         & \multicolumn{1}{c|}{92\%}       & \multicolumn{1}{c|}{2\%}         & 6\%         & \multicolumn{1}{c|}{70\%}       & \multicolumn{1}{c|}{5\%}         & 25\%        & \multicolumn{1}{c|}{89\%}       & \multicolumn{1}{c|}{3\%}         & 8\%         & \multicolumn{1}{c|}{30\%}       & \multicolumn{1}{c|}{6\%}         & 64\%        \\ \hline
\multicolumn{1}{|l|}{\textit{Unhealthy}} & \multicolumn{1}{c|}{\textit{2\%}} & \multicolumn{1}{c|}{\textit{\textless{}0.1\%}} & \textit{98\%} & \multicolumn{1}{c|}{1.3\%}      & \multicolumn{1}{c|}{0.2\%}       & 98.5\%      & \multicolumn{1}{c|}{30\%}       & \multicolumn{1}{c|}{6\%}         & 64\%        & \multicolumn{1}{c|}{96\%}       & \multicolumn{1}{c|}{1.5\%}       & 2.5         & \multicolumn{1}{c|}{40\%}       & \multicolumn{1}{c|}{1\%}         & 59\%        \\ \hline
\end{tabular}
}
\label{tab:GeneralHealthRiskPrediction}
\end{table}
\begin{table}[H]
\centering
\caption{\textbf{The percentage of \emph{apparently-healthy} patients who later develop conditions within each predicted risk group}. Among all methods (top three shown), SPHR-predicted \emph{Normal} and \emph{High} risk patients developed the fewest and most conditions, respectively, as expected.   }
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|lll|lll|}
\cline{2-10}
\multicolumn{1}{c|}{\textbf{}}                    & \multicolumn{3}{c|}{\textbf{P0 + Euclidean (Not-Transformed)}}                                             & \multicolumn{3}{c|}{\textbf{DeepPatient + Euclidean}}                    & \multicolumn{3}{c|}{\textbf{SPHR + Euclidean}}                              \\ \hline
\multicolumn{1}{|l|}{\textit{Future Diagnosis}}   & \multicolumn{1}{l|}{Normal}        & \multicolumn{1}{l|}{Lower Risk}    & \multicolumn{1}{l|}{Higher Risk} & \multicolumn{1}{l|}{Normal} & \multicolumn{1}{l|}{Lower Risk} & Higher Risk & \multicolumn{1}{l|}{Normal} & \multicolumn{1}{l|}{Lower Risk} & Higher Risk \\ \hline
\multicolumn{1}{|l|}{\textit{Cancer}}             & \multicolumn{1}{c|}{3.17\%} & \multicolumn{1}{c|}{0.92\%} & 2.83\%          & \multicolumn{1}{l|}{3.21\%}   & \multicolumn{1}{l|}{<0.1\%}          & <0.1\%           & \multicolumn{1}{l|}{1.67\%}   & \multicolumn{1}{l|}{2.85\%}       & 3.22\%        \\ \hline
\multicolumn{1}{|l|}{\textit{Diabetes}}           & \multicolumn{1}{c|}{1.26\%}          & \multicolumn{1}{c|}{1.85\%}          & 1.41\%                            & \multicolumn{1}{l|}{0.51\%}   & \multicolumn{1}{l|}{<0.1\%}          & <0.1\%           & \multicolumn{1}{l|}{0.50\%}   & \multicolumn{1}{l|}{<0.1\%}        & 4.80\%        \\ \hline
\multicolumn{1}{|l|}{\textit{Other Serious Cond}} & \multicolumn{1}{c|}{9.3\%}           & \multicolumn{1}{c|}{5.66\%}          & 9.29\%                             & \multicolumn{1}{l|}{8.77\%}   & \multicolumn{1}{l|}{4.98\%}         & 6.81\%        & \multicolumn{1}{l|}{1.47\%}   & \multicolumn{1}{l|}{8.33\%}       & 11.65\%      \\ \hline
\end{tabular}
}
\label{tab:FutureRiskPrediction}
\end{table}


    
\end{enumerate}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

